A Primal-Dual Analysis of Monotone Submodular Maximization

In this paper we design a new primal-dual algorithm for the classic discrete optimization problem of maximizing a monotone submodular function subject to a cardinality constraint achieving the optimal approximation of $(1-1/e)$. This problem and its special case, the maximum $k$-coverage problem, have a wide range of applications in various fields including operations research, machine learning, and economics. While greedy algorithms have been known to achieve this approximation factor, our algorithms also provide a dual certificate which upper bounds the optimum value of any instance. This certificate may be used in practice to certify much stronger guarantees than the worst-case $(1-1/e)$ approximation factor.

==> dual-fittings/bqs-dual-fit-deepc-buggy-old.tex <==
\section{BQS Dual Fit}
\deepc{I still have to go through this, but will probably get to it on Saturday/Sunday}

In this section we describe a dual fitting argument for a result returned from the BQS upper bound algorithm. To do so we begin with a description of the algorithm from \cite{BalkQS21}. Here we use the notation $a_i:= e \in V \mid \forall u \in V \setminus \{a_1,\cdots,a_{i-1}\}, f(e) \geq f(u)$ to refer to the element with the $ith$ highest singleton value, and $A_i:=\{a_1,\cdots,a_{i}\}$ to be the set containing the $i$ elements with the highest singleton values.
\begin{center}
	\fbox{%
		\begin{varwidth}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
			%\begin{algorithm}[H]
				%	\caption{Continuous Dual Algorithm}
				\begin{algorithmic}[1]
					\Procedure{BQS Method 3}{$f,V,k$}: 
					%\LineComment{Initialization}
					\For{$j=1$ to $k$}
					\State $i_j \gets \min \{i ~:~ f(A_i) - \sum_{\ell=1}^{j-1}v_\ell \geq f(a_i)\}$ \label{bqs:i}
					\If{$f(A_{i_j-1})-\sum_{\ell=1}^{j-1}v_\ell \geq f(a_{i_j})$} \label{bqs:if}
					%\State $i \gets i-1$
					\State $v_j \gets f(A_{i_j-1})-\sum_{\ell=1}^{j-1}v_\ell$ \label{bqs:vjif}
					\Else
					\State $v_j \gets f(a_{i_j})$ \label{bqs:else}
					\EndIf
					\EndFor
					\State \Return $\sum_{j=1}^kv_j$
					\EndProcedure
				\end{algorithmic}					
				%	\end{algorithm} 
		\end{varwidth}%
	}
\end{center}
The algorithm also terminates with $k$ indices $\{i_1, i_2, \ldots, i_k\}$. The dual is going to be supported on (at most) $2k-1$ sets, 
with the first set $S_1 = \emptyset$, and the $2k-2$ sets which occur in pairs, and we denote them as  $(L_t, R_t)$ for $2\leq t\leq k$. 
These simply are 
\[
L_t = A_{i_{t-1} - 1} ~~~\textrm{and}~~~ R_t = A_{i_{t-1}} 
\]
So, $L_2 = A_{i_1 - 1}$ and $R_2 = A_{i_1}$, $L_3 = A_{i_2 - 1}$ and $R_3 = A_{i_2}$, and so on; note that it is possible $L_t = R_{t-1}$ if $i_{t-2} = i_{t-1} - 1$. It will still be convenient to consider them as separate sets. 


One key observation about the $(v_1, \ldots, v_k)$ that we will be using is the following:
\begin{lemma}\label{lem:bqsdualfit-ko1}
	$\forall 2\leq t\leq k~:~f(L_t) ~\leq~ \sum_{\ell = 1}^{t-1} v_\ell ~\leq~ f(R_t)$
\end{lemma}
\begin{proof}
	Consider iteration $(t-1)$ and suppose Line~\ref{bqs:if} in the algorithm is true. 
	Then, $v_{t-1}$ is set in such a way that $\sum_{\ell=1}^{t-1} v_\ell = f(A_{i_{t-1} - 1}) = f(L_t)$; so the first inequality (reading left to right) is a equality and the second follows from monotonicity. If not, then $v_{t-1} = f(a_{i_{t-1}})$, and so by design the first inequality holds strictly. 
	The second inequality now holds because of the condition in Line~\ref{bqs:i}
\end{proof}
Therefore, for all $t\in [2,k]$, there exists $\lambda_t$ and $\rho_t$ such that $\lambda_t + \rho_t = 1$ and 
\[
\lambda_t f(L_t) + \rho_t f(R_t) = \sum_{\ell=1}^{t-1} v_\ell
\]

The second key observation about the BQS algorithm is the following.
\begin{lemma}\label{lem:bqsdualfit-ko2}
	Fix an element $e$. Let $t$ be the index such that $e\notin L_t$ but $e\in L_{t+1}$;
	in case, $e\notin L_k$, then define $t=k$.
	The assertion is
	\[
	\lambda_t \cdot f_{L_t}(e) + \rho_t \cdot f_{R_t}(e) \leq v_t
	\]
\end{lemma}
\begin{proof}
	Note that both $L_t\cup \{e\}$ and $R_t \cup \{e\}$ are $\subseteq L_{t+1}$, and therefore by monotonicity 
	$f_{L_t}(e) \leq f(L_{t+1}) - f(L_t)$ and $f_{R_t}(e) \leq f(L_{t+1}) - f(R_t)$
	giving 
	\[
	\lambda_t \cdot f_{L_t}(e) + \rho_t \cdot f_{R_t}(e) \leq f(L_{t+1}) - \left(\lambda_t f(L_t) + \rho_t f(R_t)\right) \leq v_t
	\]
	where the last inequality used $f(L_{t+1}) \leq \sum_{\ell=1}^t v_\ell$ and the definition of $(\lambda_t, \rho_t)$.
\end{proof}
\noindent
Now consider parameters $\tau_1, \ldots, \tau_k \in [0,1]$ which sum up to $1$; we will specify the precise values later. Using these, define the dual solution with
$\tau_{S_1} = \tau_1$ and for $2\leq t \leq k$, we let $\tau_{L_t} = \lambda_t\tau_t$ and $\tau_{R_t} = \rho_t \tau_t$. \smallskip

\noindent
First consider $\Exp_{S\sim \tau} [f(S)]$. Using the definition of $(\lambda_t, \rho_t)$, we see that this is (noting that $S_1 = \emptyset$)
\[
\sum_{t=2}^k \tau_t \cdot \left(\sum_{\ell=1}^{t-1} v_\ell \right) = \sum_{\ell=1}^k v_\ell - \sum_{\ell=1}^k v_\ell \cdot \left(\sum_{t=1}^\ell \tau_t\right)
\]
Next consider any element $e \in V$. Let $t^*$ be as defined in~\Cref{lem:bqsdualfit-ko2}. 

Then note that
\[
\Exp_{S \sim \tau} [f_S(e)] = f_{S_1}(e) + \sum_{t=2}^{t^*} \tau_t\cdot \left(\lambda_t f_{L_t}(e) + \rho_t f_{R_t}(e)\right)
\]
Now for $t \leq t^* - 1$, we will use $f_{L_t}(e), f_{R_t}(e) \leq f(e) \leq f()$

\pagebreak
We now construct the following dual solution placing $\tau$ values on $k$ different sets, $S_1,\cdots,S_k$, each corresponding to a $v$ value in the BQS solution as follows. For a given $j \in [1,k]$ we define $S_j$ to be $A_{i^*}$ in the case that $v_j$ was assigned in line~\ref{bqs:vjif} and $A_{i^*-2}$ if $v_j$ was assigned in line~\ref{bqs:else}. Additionally, given any element $e \in V$, $j_e:=\max{j \mid S_j \not\ni e}$ is the largest $S_j$ which does not contain $e$. In all cases the following observations hold:
\begin{equation}\label{eq:bqs:vj}
	\forall j \in [1,k], \quad f(S_j) \leq \sum_{\ell = 1}^jv_\ell
\end{equation}
\begin{equation}\label{eq:bqs:aj}
	\forall e \in V, \quad \forall j \leq j_e, \quad f_{S_j}(e) \leq f(e) \leq v_{j_e}
\end{equation}
Note that \cref{eq:bqs:vj} holds from line~\ref{bqs:vjif} in the case $v_j$ is assigned at that line, and lines~\ref{bqs:i} and~\ref{bqs:else} otherwise. Additionally, \cref{eq:bqs:aj} holds from the condition on line~\ref{bqs:if} and from line~\ref{bqs:else} otherwise. We are now ready to describe our dual fitting in terms of $\tau$ values:

\begin{align*}
	\alpha &= \max_{e \in V}\left(\sum_{j \in [1,k]}\left(\tau_{S_j}f_{S_j}(e)\right)\right) \\
	&= \max_{e \in V}\left(\sum_{j \in [1,j_e]}\left(\tau_{S_j}f_{S_j}(e)\right)\right)\\
	& \leq \max_{e \in V}\left(\sum_{j \in [1,j_e]}\tau_{S_j} v_{j_e}\right) & \text{from \cref{eq:bqs:aj}} \\
	& = \max_{\ell \in [1,k]}\left(\sum_{j \in [1,\ell]}\tau_{S_j}v_{\ell}\right) \\
\end{align*}
\begin{align*}
	\gamma &= \sum_{j \in [1,k]}\left(\tau_{S_j}f(S_j)\right)\\
	& \leq \sum_{j \in [1,k]}\left(\tau_{S_j}\sum_{\ell \in [1,j]}v_{\ell}\right) & \text{from \cref{eq:bqs:vj}} \\
	& = \sum_{\ell \in [1,k]}\left(v_{\ell}\sum_{j \in [\ell,k]}\tau_{S_j}\right) \\
	& = \sum_{\ell \in [1,k]}\left(v_{\ell}\left(1-\sum_{j \in [1,\ell-1]}\tau_{S_j}\right)\right) & \text{\luc{this the bug - if this sum were from 1 to $\ell$ we'd be happy}}\\
	& = \sum_{\ell \in [1,k]}\left(v_{\ell}\right) - \sum_{\ell \in [1,k]}\sum_{j \in [1,\ell-1]}\left(\tau_{S_j} v_\ell\right) \\
\end{align*}
\begin{align*}
	\dual &= \gamma + k\alpha \\
	&\leq \sum_{\ell \in [1,k]}\left(v_{\ell}\right) - \sum_{\ell \in [1,k]}\sum_{j \in [1,\ell-1]}\left(\tau_{S_j} v_\ell\right) + k\cdot\max_{\ell \in [1,k]}\left(\sum_{j \in [1,\ell]}\tau_{S_j}v_{\ell}\right)
\end{align*}
Now, note that that if 
\begin{equation}\label{eq:bqs:equality}
	\forall \ell \in [1,k], \quad \sum_{j \in [1,\ell-1]}\tau_{S_j}v_\ell = \max_{i \in [1,k]}\left(\sum_{j \in [1,i]}\tau_{S_j}v_{i}\right)
\end{equation} 
\luc{this can't possibly hold due to the LHS value when $\ell=1$ being 0}
Then $\dual \leq \sum_{\ell \in [1,k]}\left(v_{\ell}\right)$. Thus, if we assign our $\tau$ values such that \cref{eq:bqs:equality} holds, we have a proper dual fitting. Observing that $\forall i,j \in [1,k], \quad i \leq j \implies v_i \geq v_j$\footnote{One can see that $\forall j \in [1,k],\quad f(a_{j^*+1}) \leq v_j \leq f(a_j^*)$ and $\forall i,j \in [1,k],\quad i \leq j \implies i^* \leq j^*$. This implies the decreasing ordering of $v_j$}, we can make the following $\tau$ assignment of
\[\forall j \in [1,k],\quad \tau_{S_j} = \frac{v_k}{v_j} - \sum_{i \in [j-1]}\tau_{i}\]
which satisfies \cref{eq:bqs:equality}, yielding the dual fitting.


==> experiment-figs.tex <==
% \if\format I
% \section{Experimental Data}\label{sec:expdata}
% \fi
\begin{figure}[H]
	\centering
\includegraphics[width=0.9\textwidth]{data/greedycomp.png}
	\caption{Objective value comparison of greedy and primal-dual algorithms. Both algorithms perform comparatively across data set trials with the greedy algorithm often \emph{slightly} outperforming the primal-dual algorithm}
\begin{table}[H]
	\centering
	\scalebox{0.8}{
		\begin{tabular}{|c c c c c c c c|} 
			\hline
			& BA Graph & ER Graph & SBM Graph & WS Graph &  CA Roads & Facebook & Youtube\\ [0.5ex] 
			\hline\hline
			Greedy/$\dual$ & 0.9589 & 0.8839 & 0.9530 & 0.9919 & 0.9167 & 0.8212 & 0.9381\\ 
			\hline
			Primal-Dual/$\dual$ & 0.9558 & 0.8527 & 0.9397 & 0.9875 & 0.8630 & 0.8092 & 0.9378\\
			\hline
			Greedy/$\dualfit$ & 0.7530 & 0.7341 & 0.7656 & 0.8719 & 0.7645 & 0.7071 & 0.7181\\ 
			\hline
			Primal-Dual/$\dualfit$ & 0.7506 & 0.7082 & 0.7548 & 0.8678 & 0.7917 & 0.6963 & 0.7184 \\
			\hline
		\end{tabular}
	}
	\caption{Average ratios across all trials for each data set. The dual certificate from the novel primal dual algorithm often provides an approximation guaruntee in excess of 85\%, \emph{strongly} outperforming the greedy dualfit certficate described in \cref{sec:dual-fitting}.}
	\label{tab:algo}
\end{table}
% \end{figure}
% \begin{figure}[H]
	\centering
	\includegraphics[width=0.9\textwidth]{data/certificate_benchmark.png}
	\caption{Dual certificates compared to pre-existing instance specific upper bounds. The dual certificate generated from the primal-dual upper bound often outperforms all traditional benchmarks and performs comparatively to the BQS upper bound.}
	\label{fig:ub-comp}
 \end{figure}
\begin{table}[H]
	\centering
	\scalebox{0.8}{
		\begin{tabular}{|c c c c c c c c|} 
			\hline
			& BA Graph & ER Graph & SBM Graph & WS Graph &  CA Roads & Facebook & Youtube\\ [0.5ex] 
			\hline\hline
			$\dual$ & 0.9589 & 0.8839 & 0.9530 & 0.9919 & 0.9167 & 0.8212 & 0.9381\\ 
			\hline
			$\dualfit$ & 0.7530 & 0.7341 & 0.7656 & 0.8719 & 0.7645 & 0.7071 & 0.7181\\ 
			\hline
			BQS & 0.9479 & 0.8792 & 0.9782 & 0.9944 & 0.9660 & 0.8309 & 0.9342\\
			\hline
			topk & 0.8791 & 0.8545 & 0.9531 & 0.9919 & 0.9343 & 0.7965 & 0.8379\\
			\hline
			marginal & 0.7530 & 0.7341 & 0.7691 & 0.8831 & 0.7645 & 0.7071 & 0.7242\\
			\hline
			curvature & 0.6321 & 0.6321 & 0.6321 & 0.6321 & 0.6321 & 0.7446 & 0.8226\\
			\hline
		\end{tabular}
	}
	\caption{Average greedy approximation ratio across all trials for each upper bound. The dual certificate and the BQS certificate outperform traditional methods, often providing an approximation guarantee well over 85\%.}
	\label{tab:bounds}
\end{table}
% \end{figure}
\begin{figure}[H]
	\centering
	\includegraphics[width=0.9\textwidth]{data/timetrials.png}
	\caption{Runtimes of primal-dual, greedy, and greedy+BQS algorithms. The primal-dual algorithm often runs slightly slower than the greedy algorithm, but beats out the greedy algorithm combined with a BQS upper bound calculation.}
\end{figure}

==> expt-ipco.tex <==
\section{Experimental Findings}\label{sec:expt-ipco}
%deepc: this is copy paste from \arxiv{} of section 3: need to make sure this is the same both places.

In the following table, we also give numerical values of the ratio of the greedy solution and the dual solution; closer to $1$ is better. The various columns 
are our submodular functions and the number is the average taken over all $k$'s. As one can see $\primdual$ and $\bqs$ often provide an approximation guarantee  well over 85\%.

\begin{table}[H]
	\centering
	\scalebox{0.9}{
		\begin{tabular}{|c c c c c c c c|} 
			\hline
			& BA Graph & ER Graph & SBM Graph & WS Graph &  CA Roads & Facebook & Youtube\\ [0.5ex] 
			\hline\hline
			$\primdual$ & 0.9589 & 0.8839 & 0.9530 & 0.9919 & 0.9167 & 0.8212 & 0.9381\\ 
			\hline
			$\greedydual$ & 0.7530 & 0.7341 & 0.7656 & 0.8719 & 0.7645 & 0.7071 & 0.7181\\ 
			\hline
			$\bqs$ & 0.9479 & 0.8792 & 0.9782 & 0.9944 & 0.9660 & 0.8309 & 0.9342\\
			\hline
			%			topk & 0.8791 & 0.8545 & 0.9531 & 0.9919 & 0.9343 & 0.7965 & 0.8379\\
			%			\hline
			%			marginal & 0.7530 & 0.7341 & 0.7691 & 0.8831 & 0.7645 & 0.7071 & 0.7242\\
			%			\hline
			%			curvature & 0.6321 & 0.6321 & 0.6321 & 0.6321 & 0.6321 & 0.7446 & 0.8226\\
			%			\hline
		\end{tabular}
	}
	%	\caption{Average greedy approximation ratio across all trials for each upper bound. The dual certificate and the BQS certificate outperform traditional methods, often providing an approximation guarantee well over 85\%.}
	%	\label{tab:bounds}
\end{table}

The following figure shows the comparison of the greedy solution with the primal solution returned by our primal-dual algorithm.
As can be see, the performance of the primal algorithm almost matches that of the greedy algorithm, although the latter
often \emph{slightly} outperforms the former, with the primal-dual algorithm exhibiting a maximum deviation of 8.1\% lower than greedy across all trials.

\includegraphics[width=0.9\textwidth]{data/greedycomp.png}

The following figure shows the runtimes of our primal-dual algorithm, the (naive) implementation of the greedy algorithm, and the ``Method 4'' of~\cite{BalkQS21} which returns $\bqs$.
The primal-dual algorithm often runs slightly slower than the greedy algorithm, but often beats the BQS upper bound calculation algorithm. Note that this method needs to run the greedy algorithm
and then run the ``Method 3'' of~\cite{BalkQS21} (see~\Cref{sec:bqs-dualfit} for more on this algorithm).
%\begin{figure}[H]
	%	\centering
	\includegraphics[width=0.9\textwidth]{data/timetrials.png}
	%	\caption{Runtimes of primal-dual, greedy, and greedy+BQS algorithms. The primal-dual algorithm often runs slightly slower than the greedy algorithm, but beats out the greedy algorithm combined with a BQS upper bound calculation.}
	%\end{figure}
%
%We compare our $\dual$~and $\dualfit$~certificates (with $\dualfit$ being derived from \Cref{sec:dual-fitting}) as instance-specific upper bounds to the following benchmark upper bound techniques. All implementations of these benchmarks follow the methods described by Balkanski \etal~\cite{BalkQS21}. \\
%\emph{Topk}: This benchmark gives a simplistic upper bound by taking the best $k$ elements and summing their singleton values. \\
%\emph{Marginal}: The marginal technique is described by the taking the min over all $i,j \in [k]$ of the following bound: \[\ipco{\small}\forall i<j<k, \opt \leq \frac{f(S_j)-(1-1/k)^{j-i}f(S_i)}{1-(1-1/k)^{j-i}}\]
%\emph{Curvature}: This benchmark uses the fact that the greedy algorithm actually has a worst case approximation factor of $\frac{1-e^{-c}}{c}$ where the ``curvature'', $c:=\min_{S\in 2^V, u \in V\setminus S}{\frac{f_{S}(u)}{f(u)}}$, is a measure of how close to additive $f$ is \cite{ConfC84}. In order to quickly estimate the curvature of $f$ in polynomial time, we implement an approximation of this bound via the methods described by Balkanski \etal~\cite{BalkQS21}. \\
%\emph{BQS}: This is the novel upper bound introduced by Balkanski~\etal~in 2021. It represents a significant increase in observed performance over the above benchmarks, and serves as our state of the art to which we can compare our $\dual$~upper bound.\arxiv{\input{experiment-figs}}
%\paragraph{Discussion of Results} In general, we found that the primal-dual algorithm does not provide much additional benefits with regards to its primal solution - it performs comparably to the greedy algorithm with a slower run time guarantee and similar experimental run time. Where this algorithm scheme instead provides results is in its dual certificate. Here we observe it outperforms all traditional benchmarks and performs comparably to the BQS certificate while exhibiting a similar, if not better, experimental runtime than the combined greedy and BQS certificate algorithms. Additionally, the certificate generated from the primal dual algorithm comes with an optimal worst-case performance guarantee of $1-\frac{1}{e}$ with respect to the primal-dual solution while the BQS certificate is only able to guarantee a worst-case bound of $\frac{1}{2}$ with respect to the greedy solution. The strong experimental performance combined with a fast experimental run time and improved worst-case guarantee lead us to believe the primal-dual algorithm with dual certificate has legitimate utility for some applications and should be studied further in task-specific contexts.

==> illus-ipco.tex <==
\section{Pseudocode, Illustrative Example, and Discretization}\label{sec:illus-ipco}
The full pseudocode of the algorithm is described below. 
\begin{center}
	\footnotesize{
		\fbox{%
			\begin{varwidth}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
				%\begin{algorithm}[H]
					%	\caption{Continuous Dual Algorithm}
					\begin{algorithmic}[1]
						\Procedure{MSM Primal-Dual}{$f,V,k$}: 
						%\LineComment{Initialization}
						\State $i\eq 1$; $\calA^{(i)} \gets \{\emptyset\}$; $\ALG^{(i)} \leftarrow \emptyset$; $\tau_\emptyset \gets 1$; $\gamma \gets 0$
						\State $\forall j \in V, \beta_j \gets f(\{j\}), \dt{\beta}(j) \gets 0$; $\alpha \gets \max_{j \in V}f(j)$; $\dt{\alpha} \gets 0$; $\dt{\gamma} \gets 0$
						\State $T \gets \{{j \in V \mid \beta_j = \alpha}\}$ 
						% \State $\ALG \leftarrow \emptyset$ 
						% \Comment{Current pick set}
						\While{$i < k+1$}
						\While{$k\dt{\alpha} + \dt{\gamma} < 0$} %\Comment{We are decreasing dual}
						\LineComment{\sc Make Dual Progress}
						\State $\dt{\tau_{\ALG^{(i)}}} \eq 1 - \tau_{\ALG^{(i)}}$. \label{alg:mdp-first}
						\State $\dt{\tau_{S}} \eq - \tau_{S}$, $\forall S\in \calA^{(i)}\setminus \ALG^{(i)}$.
						\State $\dt{\beta}_j \eq f_{\ALG^{(i)}}(j) - \beta_j$, $\forall j\in V$. 
						\State $\dt{\gamma} \gets f(\ALG^{(i)}) - \gamma$
						\State $T \gets \{{j \in V \mid \beta_j = \alpha}\}$ \Comment{$j$'s may leave and enter $T$ as we change $\alpha$, $\beta_j$'s}
						\State $\dt{\alpha} \gets \max_{j\in T}(\dt{\beta}_j)$ \label{alg:mdp-last}
						\EndWhile
						\LineComment{\sc Make Primal Pick}
						\State $p_i \eq \arg \max_{j\in T} \dt{\beta_j}$; $\ALG^{(i+1)} \eq \ALG^{(i)} \cup p_i$;  $\calA^{(i+1)} \eq \calA^{(i)} \cup \ALG^{(i+1)}$ \label{alg:16}
						\State $\dt{\gamma} \eq f(\ALG^{(i+1)}) - \gamma$. \label{alg:17}
						\State $\dt{\beta_j} \eq f_{\ALG^{(i+1)}}(j) - \beta_j$, $\forall j\in V$. 
						\State $\dt{\alpha} \eq \max_{j\in T} \dt{\beta_j}$; $i\eq i+1$. \label{alg:19}
						\EndWhile
						\State \Return $\ALG^{(k+1)}$, $(\alpha, \tau_S~:~S\in \calA^{(k+1)})$.
						\EndProcedure
					\end{algorithmic}					
					%	\end{algorithm} 
			\end{varwidth}%
		}
	}
\end{center}
As written, lines~\ref{alg:mdp-first} to~\ref{alg:mdp-last} continuously checks the while-loop condition. In~\Cref{sec:discrete} we describe how to implement this efficiently.
In short, the only times we need to be careful is when a new element enters the set $T$ and these ``times'' can be found via solving simple ordinary differential equations. 

\input{illus-ex}
\input{discretization}

==> ipco/expermient-figs-ipco.tex <==
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth,height=0.25\textheight]{data/greedycomp.png}
	\caption{Objective value comparison of greedy and primal-dual algorithms. Both algorithms perform comparatively across data set trials with the greedy algorithm often \emph{slightly} outperforming the primal-dual algorithm}
\includegraphics[width=\textwidth,height=0.25\textheight]{data/certificate_benchmark.png}
	\caption{Dual certificates compared to pre-existing instance specific upper bounds. The dual certificate generated from the primal-dual upper bound often outperforms all traditional benchmarks and performs comparatively to the BQS upper bound.}
	\includegraphics[width=\textwidth,height=0.25\textheight]{data/timetrials.png}
	\caption{Runtimes of primal-dual, greedy, and greedy+BQS algorithms. The primal-dual algorithm often runs slightly slower than the greedy algorithm, but beats out the greedy algorithm combined with a BQS upper bound calculation.}
\end{figure}

==> ipco/starter-ipco.tex <==
\usepackage{amsmath, amssymb}
\usepackage{ifthen}
\usepackage{soul}
% \usepackage{fullpage, prettyref}
\usepackage{fancyhdr}
%\usepackage{palatino}
\usepackage{graphicx}
\usepackage{marvosym}
\usepackage{ifthen}
\usepackage{algorithm}

\newcommand{\Lim}{\lim}

\usepackage{mdframed}
\usepackage{url}
% \usepackage{fullpage, prettyref}
\usepackage{boxedminipage}
\usepackage{wrapfig}
\usepackage{ifthen}
\usepackage{color,xcolor}
\usepackage{transparent}
\usepackage{enumitem}
\usepackage{varwidth}
\usepackage[pagebackref,colorlinks=true,pdfpagemode=none,urlcolor=blue,linkcolor=blue,citecolor=violet,pdfstartview=FitH]{hyperref}
\usepackage[noabbrev,nameinlink]{cleveref}


%\def\bar{\overline}


\def\plus{{\tt (+)}}
\def\2plus{{\tt (++)}}
\def\3plus{{\tt (+++)}}
\def\4plus{{\tt (++++)}}
\def\5plus{{\tt (+++++)}}






\usepackage{ifthen}
\usepackage{soul}
% \usepackage{fullpage, prettyref}
\usepackage{fancyhdr}
\usepackage{color,xcolor}

% \usepackage{times}
%\usepackage{palatino}
\usepackage{graphicx}
\usepackage{marvosym}
\usepackage{ifthen}
\usepackage{algorithm}

\usepackage[noend]{algpseudocode}
\algrenewcomment[1]{\(\triangleright\) {\small{\emph{\color{blue} #1}}}}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) \emph{\color{blue} #1}}
\algnewcommand{\Invariant}[1]{\State \(\triangleright\) \emph{\color{red} #1}}
%\newcommand{\Lim}{\lim}


% \usepackage{amsmath, amssymb, amsthm}
\usepackage{url}
% \usepackage{fullpage, prettyref}
%\usepackage{pstricks,pst-node,pst-text}
\usepackage{boxedminipage}
\usepackage{wrapfig}
\usepackage{ifthen}

\usepackage{transparent}
\usepackage{enumitem}
\usepackage{varwidth}



%\theoremstyle{definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{claim}{Claim}
% \newtheorem{corollary}{Corollary}
% \newtheorem{definition}{Definition}
% \newtheorem{proposition}{Proposition}
\newtheorem{fact}{Fact}
% \newtheorem{example}{Example}
% \newtheorem{exercise}{Problem}
\newtheorem{drill}{Exercise}
\newtheorem{assumption}{Assumption}
\newtheorem{observation}{Observation}

\newcommand{\comment}[1]{\textsl{\color{brown} \small[#1]}\marginpar{\tiny\textsc{\color{red} To Do!}}}
\newcommand{\ignore}[1]{}



\def\plus{{\tt (+)}}
\def\2plus{{\tt (++)}}
\def\3plus{{\tt (+++)}}
\def\4plus{{\tt (++++)}}
\def\5plus{{\tt (+++++)}}




% \newenvironment{proofof}[1]{\smallskip\noindent{\bf Proof of #1:}}%
% {\hspace*{\fill}$\Box$\par}

% \setlength{\oddsidemargin}{0pt}
% \setlength{\evensidemargin}{0pt}
% \setlength{\textwidth}{6.5in}
% \setlength{\topmargin}{0in}
% \setlength{\textheight}{8.5in}
% \newlength{\algobox}
% \setlength{\algobox}{6.5in}

\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\xor}{\oplus}
\newcommand{\range}{\mathrm{range}}

\newcommand{\OPT}{\mathtt{OPT}}
\newcommand{\ALG}{\mathtt{ALG}}
\newcommand{\opt}{\mathtt{opt}}
\newcommand{\cost}{\mathtt{cost}}
\newcommand{\alg}{\mathsf{alg}}
\newcommand{\spn}{\mathsf{span}}
\newcommand{\row}{\mathsf{row}}
\newcommand{\supp}{\mathsf{supp}}

\newcommand{\APX}{\ensuremath{\mbox{APX}}}
\newcommand{\apx}{\ensuremath{\mbox{apx}}}


\def\Math{{\color{red} \Libra}}







\renewcommand{\theenumi}{\alph{enumi}}

%%%%%%%%%%%%%%%%%%%%   SHORTCUTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Calligraphic Letters
\newcommand{\script}[1]{\mathcal{#1}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}


%MathBB letters
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\ZZ}{\mathbb{Z}}


%Mathbold letters
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bmm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\bI}{\mathbf{I}}

\newcommand{\bone}{\mathbf{1}}
\newcommand{\bzero}{\mathbf{0}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bG}{\boldsymbol{G}}

\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}



%Commonly used text in mathmode
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\littlesum}{\mathop{{\textstyle \sum}}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}

\newcommand{\barx}{\overline{x}}
\newcommand{\bary}{\overline{y}}

\newcommand{\lee}{\leqslant}
\newcommand{\gee}{\geqslant}
\newcommand{\ceil}[1]{{\left\lceil{#1}\right\rceil}}
\newcommand{\floor}[1]{{\left\lfloor{#1}\right\rfloor}}

\DeclareMathOperator*{\Exp}{\ensuremath{{\mathbf{Exp}}}}
\DeclareMathOperator*{\Var}{\ensuremath{{\mathbf{Var}}}}
\DeclareMathOperator*{\Prob}{\ensuremath{\mathbf{Pr}}}
\renewcommand{\Pr}{\Prob}
\newcommand{\EX}{\Exp}
\newcommand{\Ex}{\Exp}
\newcommand{\bigO}[1]{\ensuremath{O\Paren{#1}}}

\newcommand{\prob}[1]{\Pr\paren{#1}}
\newcommand{\expect}[1]{\Exp\bracket{#1}}
\newcommand{\var}[1]{\textnormal{Var}\bracket{#1}}
\newcommand{\eexp}[1]{\exp\paren{#1}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1 \right\}}}

\newcommand{\tvd}[2]{\ensuremath{\norm{#1 - #2}_{tvd}}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\Paren}[1]{\Big(#1\Big)}
\newcommand{\Bracket}[1]{\Big[#1\Big]}
\newcommand{\bracket}[1]{\left[#1\right]}
\newcommand{\paren}[1]{\ensuremath{\left(#1\right)}\xspace}
\newcommand{\card}[1]{\left\vert{#1}\right\vert}
\newcommand{\Ot}{\ensuremath{\widetilde{O}}}
\newcommand{\Omgt}{\ensuremath{\widetilde{\Omega}}}
\newcommand{\half}{\ensuremath{{1 \over 2}}}


\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\psdgeq}{\succcurlyeq}
\newcommand{\eqdef}{\overset{\mathrm{\tiny def}}{=\joinrel=}}
\newcommand{\grad}{\nabla}
\newcommand{\minimize}{\mathrm{minimize}\quad}
\newcommand{\maximize}{\mathrm{maximize}\quad}
%% Hyper-linked References
%\newcommand{\Sec}[1]{\hyperref[sec:#1]{\S\ref*{sec:#1}}} %section
%\newcommand{\Eqn}[1]{\hyperref[eq:#1]{(\ref*{eq:#1})}} %equation
%\newcommand{\Fig}[1]{\hyperref[fig:#1]{Fig.\,\ref*{fig:#1}}} %figure
%\newcommand{\Tab}[1]{\hyperref[tab:#1]{Tab.\,\ref*{tab:#1}}} %table
%\newcommand{\Thm}[1]{\hyperref[thm:#1]{Theorem\,\ref*{thm:#1}}} %theorem
%\newcommand{\Fact}[1]{\hyperref[fact:#1]{Fact\,\ref*{fact:#1}}} %fact
%\newcommand{\Lem}[1]{\hyperref[lem:#1]{Lemma\,\ref*{lem:#1}}} %lemma
%\newcommand{\Prop}[1]{\hyperref[prop:#1]{Prop.~\ref*{prop:#1}}} %property
%\newcommand{\Cor}[1]{\hyperref[cor:#1]{Corollary~\ref*{cor:#1}}} %corollary
%\newcommand{\Conj}[1]{\hyperref[conj:#1]{Conjecture~\ref*{conj:#1}}} %conjecture
%\newcommand{\Def}[1]{\hyperref[def:#1]{Definition~\ref*{def:#1}}} %definition
%\newcommand{\Alg}[1]{\hyperref[alg:#1]{Alg.~\ref*{alg:#1}}} %algorithm
%\newcommand{\Ex}[1]{\hyperref[ex:#1]{Ex.~\ref*{ex:#1}}} %example
%\newcommand{\Clm}[1]{\hyperref[clm:#1]{Claim~\ref*{clm:#1}}} %example
%
%\renewcommand{\Re}{\mathbf{R}}

%%%%%%%%%%%%
%\newcommand{\OPT}{\mathtt{OPT}}
%\newcommand{\ALG}{\mathtt{ALG}}
%\newcommand{\opt}{\mathtt{opt}}
%\newcommand{\cost}{\mathtt{cost}}
%\newcommand{\alg}{\mathsf{alg}}
%\newcommand{\spn}{\mathsf{span}}
%\newcommand{\row}{\mathsf{row}}
%\newcommand{\supp}{\mathsf{supp}}
%
%\newcommand{\APX}{\ensuremath{\mbox{APX}}}
%\newcommand{\apx}{\ensuremath{\mbox{apx}}}



%%%%%%%%%%%%%%%
\newcommand{\etal}{{\it et al.\,}}
\newcommand{\goodetal}{{\it et al.\/}}


\newcommand\dom{\mathbf{dom}}
\newcommand\epi{\mathbf{epi}}
\renewcommand\st{\quad\mathrm{~s.~t.~}\quad}
\newcommand\rand{\mathsf{rand}}
\newcommand{\eq}{\leftarrow}

% \newcommand{\remark}[1]{\begin{mdframed}[backgroundcolor=yellow!10,topline=false,bottomline=false,leftline=false,rightline=false] 
% 		{\bf Remark: }{\em #1} 
% \end{mdframed}}

\newcommand{\summ}[1]{\begin{mdframed}[backgroundcolor=orange!10,topline=false,bottomline=false,leftline=false,rightline=false] 
		{\bf Summary: }{\em #1} 
\end{mdframed}}

\newcommand{\todo}[1]{ \begin{mdframed}[backgroundcolor=teal!10,topline=false,bottomline=false,leftline=false,rightline=false] 
		{\bf Ponder This:}{\em #1}
\end{mdframed}}

% \newcommand{\problem}[2]{\begin{mdframed}[backgroundcolor=blue!05,topline=false,bottomline=false,leftline=false,rightline=false] 
% 		{\underline{{\sc #1}}} \\
% 		#2 
% \end{mdframed}}

\newcommand{\thingstoadd}[1]{\begin{mdframed}[backgroundcolor=red!10,topline=false,bottomline=false,leftline=false,rightline=false] 
		{\bf Things to add: }{\em #1} 
\end{mdframed}}

\newenvironment{thm}{
	\begin{mdframed}[backgroundcolor=gray!20,topline=false,bottomline=false,leftline=false,rightline=false]\begin{theorem}
		}{
		\end{theorem}
	\end{mdframed}
}

\newcommand{\deepc}[1]{{\color{red} {\bf deepc:} #1}}
\newcommand{\luc}[1]{{\color{red} {\bf luc:} #1}}


==> primal-dual-card.tex <==
\section{A Primal-Dual Algorithm under the Cardinality Constraint}\label{sec:2}
% \subsection{The Primal, the Dual, and the Primal-Dual Algorithm}

As mentioned in the introduction, the primal formulation of \msm~ is inspired by Wolsey's formulation~\cite{Wolsey82} for the submodular set cover problem.
We begin with this and its dual. 

\begin{minipage}{0.46\textwidth}
	\begin{alignat}{6}
		\lp:=&&\max~~~~\lambda~&&~&\tag{\sf{primal}} \label{eq:primal} \\
		&&\sum_{j \in V} x_j &~=~ && k~&\tag{P1}\label{eq:p1}\\
		&&\lambda - \sum_{j \in V} f_{S}(j)x_j &~\leq~ && f(S), && ~\forall S \subseteq V \tag{P2}\label{eq:p2}\\
		&&x_j &~\geq~&& 0, && ~\forall j\in V \notag
	\end{alignat}
\end{minipage} ~~~\vline
\begin{minipage}{0.45\textwidth}
	\begin{alignat}{6}
		\min~   &&~k\alpha + \sum_{S\subseteq V}\tau_S f(S)  &=:&& \dual \notag\\
		&&\alpha - \sum_{S\subseteq V}\tau_S f_{S}(j) &~\geq~ && 0,~ \forall j \in V \tag{D1} \label{eq:d1}\\
		&& \sum_{S\subseteq V} \tau_S &~=~&& 1 \tag{D2} \label{eq:d2}\\
		&& \tau_S &~\geq~&& 0, ~\forall S\subseteq V \tag{D3} \label{eq:d3}
	\end{alignat}
\end{minipage}
\vspace{1ex}

\noindent
The following claim is similar to Proposition 2 in~\cite{Wolsey82}.
\begin{claim}
	For any instance of \msm, $\lp \geq \opt$.
\end{claim}
\begin{proof}
	Let $S^*$ be an optimal solution, and consider the following solution to the primal linear program: $x_j = 1$ for $j\in S^*$ and $x_j = 0$ for $j\in V\setminus S^*$, and $\lambda = f(S^*)$.
	We claim that $(x,\lambda)$ is a feasible solution which would prove the claim. Clearly, $\sum_{j\in V} x_j = |S^*| = k$. Fix $S\subseteq V$ and note
	\begin{alignat}{2}
		f(S) + \sum_{j \in V} f_{S}(j)x_j ~=~ f(S) + \sum_{j\in S^*} f_S(j) ~\underbrace{\geq}_{\text{\Cref{clm:fnw}}}~ f(S^*) = \lambda \notag
	\end{alignat}
	rearranging which proves feasibility.
\end{proof}
\noindent
Indeed, one can see that when restricted to $x_j\in \{0,1\}$ the linear program's optimum value equals $\opt$. 
%Given a feasible solution $(x,\lambda)$ to \eqref{eq:primal}, it is not too hard to design a randomized rounding algorithm which returns a set $R$ with $\Exp[f(R)] \geq (1-1/e)\cdot \lambda$, thus showing that the integrality gap of the LP is bounded by this factor. In fact, we never use submodularity (or monotonicity) in this argument; indeed, these facts are only used in the previous claim.
%Unfortunately, it is not clear how to solve the above LP. Indeed, we can show that checking whether \eqref{eq:p2} is satisfied by a given $(x,\lambda)$ may take exponentially many queries to $f$. We include a discussion of this in~\Cref{sec:notes-on-primal}. \medskip


The dual program has a variable $\alpha$ corresponding to \eqref{eq:p1} and a variable $\tau_S$ for every subset $S\subseteq V$ corresponding to \eqref{eq:p2}. Note that \eqref{eq:d2} and \eqref{eq:d3} imply that $\tau$'s form a probability distribution over the sets. The dual objective is $k\alpha$ plus the expected value of a set drawn from this $\tau$-distribution. 
Although the dual has exponentially many variables, our primal-dual algorithm will maintain a polynomially many (in fact $k+1$ many) subsets with positive $\tau$.
Indeed, it is not too hard to give a dual-fitting analysis of the greedy algorithm using the above dual. We include a discussion of this in~\Cref{sec:dual-fitting}, and the math is similar to the proof given in~\cite{NemhWF78}.  In the remainder of this section we focus on the primal-dual algorithm. 

\subsection{Primal-Dual Algorithm}
\todo{ Improve algorithm explanation, integrate appendix examples}
As is often the case, the primal-dual algorithm is best understood as a continuous-time algorithm. We try to modify the dual variables at certain rates so as to maintain dual feasibility and {\em decrease} the dual objective value. When we cannot decrease the dual any further, at that juncture we make a primal choice and pick an element in our $\ALG$ set, and modify dual variables forced by this change. 
We continue this process till we can't pick any more items in $\ALG$. We now explain the details of this process.
To do so, we begin with some definitions which will remain invariant throughout the algorithm. %We use a superscript indexed by $t$ (for time) to underscore this. 
\begin{itemize}[noitemsep]
	\item We maintain a {\em chain} of subsets $\calA$ and $\tau_S > 0$ only for $S\in \calA$. $\ALG$ is the maximal set of $\calA$.
	\item $\sum_{S\in \calA} \tau_S = 1$.
	\item We maintain variables $\gamma := \sum_{S\in \calA} \tau_S f(S)$ and $\forall j \in V$,  $\beta_j := \sum_{S \in \calA} \tau_S f_{S}(j)$.
	\item $\alpha := \max_{j\in V} \beta_j$ and let $T := \{j\in V: \alpha = \beta_j\}$ be the ``tight'' elements. This set is never non-empty.
	\item $\dual := k\alpha + \gamma$.
\end{itemize}
Note that if we maintain the above properties, $(\alpha, \tau_S)$ forms a feasible dual solution with objective value $\dual$. 
%Whenever clear, we remove the superscript $(t)$ from the various variables to avoid clutter.
We initially set  $\calA = \{\emptyset\}$ and $\tau_\emptyset = 1$. Note that all other variables are defined by these. 
In particular, $\gamma = 0$, $\beta_j = f(\{j\})$ for all $j\in V$, $\alpha = \max_{j\in V} f(\{j\})$, $T = \{j\in V:f(j) = \alpha\}$, and 
$\dual = k\alpha$.

\medskip

The algorithm has two phases. The {\sc Make Dual Progress} phase modifies the dual variables $\tau_S$ which leads to modifications of all other variables as per the above definition.
To begin with, we describe a continuous time version of this phase using the rate of changes of these variables. We denote these rates by adding a dot above the variable name.
The dual modification phase is run {\em only if} the dual decreases. 
%Otherwise, it runs the {\sc Make Primal Pick} phase where it picks an element to the $\ALG$ set and modifies the chain $\cA$.
%This phase does not change any dual variables, but it does change the rates for the next make dual progress phase. We give some details of the dual modification phase.

\begin{itemize}
	\item We set $\dt{\tau_{\ALG}} = 1 - \tau_{\ALG}$ and $\dt{\tau_S} = - \tau_S$ for all other $S\in \calA \setminus \ALG$. That is, we try and increase $\tau_{\ALG}$ and decrease all other $\tau_S$'s
	in the chain $\cA$.
	\item The change in $\tau$-variables leads to changes in all other variables. In particular, the $\gamma$ variable changes as follows.
	\begin{equation}\label{eq:gamma-change}
		\dt{\gamma} = (1 - \tau_{\ALG})f(\ALG) - \sum_{S\in \calA\setminus \ALG} \tau_S f(S) = f(\ALG) - \gamma
	\end{equation}			
	Note $f$ is monotone, this quantity will be non-negative, and thus we increase the $\gamma$ variable over time. 
	
	The $\beta_j$'s change as follows.
	\begin{equation}\label{eq:beta-change}
		\forall j\in V,~~~ \dt{\beta_j} = (1 - \tau_{\ALG})f_\ALG(j) - \sum_{S\in \calA\setminus \ALG} \tau_S f_S(j) =  f_\ALG(j) - \beta_j
	\end{equation}
	Note that when $f$ is submodular $f_S(j) \geq f_\ALG(j)$ for all $S\in \calA$ since $\calA$ is a chain, and thus $\dt{\beta_j}$ will be non-positive. That is, these variables decrease in value.
	
	The $\alpha$ variables changes as follows.
	\begin{equation}\label{eq:alpha-change}
		\dt{\alpha} = \max_{j\in T} \dt{\beta_j}
	\end{equation}
	The rate of change of $\alpha$ is dictated by the highest rate of $\beta_j$ change among the tight elements. Again, when $f$ is submodular these $\dt{\beta_j}$'s are negative, and thus we are going to decrease the value of $\alpha$. 
	However, note that as we keep changing $\alpha$'s and $\beta_j$'s, the set $T$ may change, and in particular a new element may appear in $T$ and lead to a different $\dt{\alpha}$. We need to keep track of this. 
	
	\item Once $\dt{\gamma}$ and $\dt{\alpha}$ are defined, we see that $\dt{\dual} = k\dt{\alpha} + \dt{\gamma}$. We only do the changes to the previous steps as long as $\dt{\dual} < 0$. Otherwise, we stop this dual-modification phase. At the beginning, note that $\dt{\gamma} = 0$, $\dt{\beta_j} = 0$, and $\dt{\alpha} = 0$ implying $\dt{\dual} = 0$. Therefore, the dual-modification phase does not run at the beginning, and we move to the primal-choice phase. 
\end{itemize}

When we cannot decrease the dual objective, we make a primal pick. We
consider the set of tight elements at this time, $T^{(i)} = \{j\in V~:~ \beta^{(i)}_j = \alpha^{(i)}\}$ and pick $p_i := \arg \max_{j\in T^{(i)}} \dt{\beta^{(i)}_j}$.
That is, $p_t$ is the element whose $\beta^{(i)}_j$ value was dropping at the rate of $\alpha^{(i)}$. 
We modify $\ALG^{(i+1)} = \ALG^{(i)} \cup \{p_i\}$ and define $\calA^{(i+1)} = \calA^{(i)} \cup \ALG^{(i+1)}$. The process then moves back to the dual-modification phase. 
Note that since the chain $\calA$ and the set $\ALG$ have changed, all the rates change, and therefore it is possible that the dual can be dropped. 
The above two dual-primal processes continue till we pick $k$ elements in $\ALG$ at which point we terminate. The full pseudocode of the algorithm is described below.

%\begin{minipage}{0.5\textwidth}
	%\begin{mdframed}[backgroundcolor=purple!10,topline=false,bottomline=false,leftline=false,rightline=false] 
		\begin{center}
			\fbox{%
				\begin{varwidth}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
					%\begin{algorithm}[H]
						%	\caption{Continuous Dual Algorithm}
						\begin{algorithmic}[1]
							\Procedure{MSM Primal-Dual}{$f,V,k$}: 
							%\LineComment{Initialization}
							\State $i\eq 1$; $\calA^{(i)} \gets \{\emptyset\}$; $\ALG^{(i)} \leftarrow \emptyset$; $\tau_\emptyset \gets 1$; $\gamma \gets 0$
							\State $\forall j \in V, \beta_j \gets f(\{j\}), \dt{\beta}(j) \gets 0$; $\alpha \gets \max_{j \in V}f(j)$; $\dt{\alpha} \gets 0$; $\dt{\gamma} \gets 0$
							\State $T \gets \{{j \in V \mid \beta_j = \alpha}\}$ 
							% \State $\ALG \leftarrow \emptyset$ 
							% \Comment{Current pick set}
							\While{$i < k+1$}
							\While{$k\dt{\alpha} + \dt{\gamma} < 0$} %\Comment{We are decreasing dual}
							\LineComment{\sc Make Dual Progress}
							\State $\dt{\tau_{\ALG^{(i)}}} \eq 1 - \tau_{\ALG^{(i)}}$. \label{alg:mdp-first}
							\State $\dt{\tau_{S}} \eq - \tau_{S}$, $\forall S\in \calA^{(i)}\setminus \ALG^{(i)}$.
							\State $\dt{\beta}_j \eq f_{\ALG^{(i)}}(j) - \beta_j$, $\forall j\in V$. 
							\State $\dt{\gamma} \gets f(\ALG^{(i)}) - \gamma$
							\State $T \gets \{{j \in V \mid \beta_j = \alpha}\}$ \Comment{$j$'s may leave and enter $T$ as we change $\alpha$, $\beta_j$'s}
							\State $\dt{\alpha} \gets \max_{j\in T}(\dt{\beta}_j)$ \label{alg:mdp-last}
							\EndWhile
							\LineComment{\sc Make Primal Pick}
							\State $p_i \eq \arg \max_{j\in T} \dt{\beta_j}$; $\ALG^{(i+1)} \eq \ALG^{(i)} \cup p_i$;  $\calA^{(i+1)} \eq \calA^{(i)} \cup \ALG^{(i+1)}$ \label{alg:16}
							\State $\dt{\gamma} \eq f(\ALG^{(i+1)}) - \gamma$. \label{alg:17}
							\State $\dt{\beta_j} \eq f_{\ALG^{(i+1)}}(j) - \beta_j$, $\forall j\in V$. 
							\State $\dt{\alpha} \eq \max_{j\in T} \dt{\beta_j}$; $i\eq i+1$. \label{alg:19}
							\EndWhile
							\State \Return $\ALG^{(k+1)}$, $(\alpha, \tau_S~:~S\in \calA^{(k+1)})$.
							\EndProcedure
						\end{algorithmic}					
						%	\end{algorithm} 
				\end{varwidth}%
			}
		\end{center}
		As written, lines~\ref{alg:mdp-first} to~\ref{alg:mdp-last} continuously checks the while-loop condition. In~\Cref{sec:discrete} we describe how to implement this efficiently.
		In short, the only times we need to be careful is when a new element enters the set $T$ and these ``times'' can be found via solving simple ordinary differential equations.
		
		\subsection{Analysis}
		
		The final $(\alpha, \tau_S)$'s form a feasible dual with objective value equal to $\dual = k\alpha + \gamma$. We now show that $f(\ALG^{(k+1)}) \geq \eta_k \cdot (k\alpha + \gamma)$ where $\eta_k = 1 - \left(1 - \frac{1}{k}\right)^k$. 
		\begin{mdframed}[backgroundcolor=gray!20,topline=false,bottomline=false,leftline=false,rightline=false] 
			\begin{theorem}
				The {\sc MSM Primal-Dual} algorithm returns a set $\ALG^{(k+1)}$ and a feasible dual solution $\tau$ with objective $\dual$ with the property
				\[
				f(\ALG^{(k+1)}) \geq \left(1 - \left(1 - \frac{1}{k}\right)^k \right) \cdot \dual
				\]
			\end{theorem}
		\end{mdframed}
		\begin{proof}
			To this end, fix time just {\em before} the $i$th item $p_i$ is picked, 
			%let $\alpha^{(t)}$ be the value of $\alpha$ at this time. 
			In what follows, all the other variables and their rates are precisely at this time.
			Let $\Delta^{(i)}$ refer to the increase in $f(\cdot)$ from picking $p_i$, that is, 
			\[
			\Delta^{(i)} := f_{\ALG^{(i)}} (p_i)
			\] 
			Now observe that 
			\begin{equation}\label{eq:main}
				f_{\ALG^{(i)}}(p_i) \geq \beta_{p_i} - \frac{\dt{\gamma}}{k}
			\end{equation}
			The reason is $p_i = \arg \max_{j\in T} \dt{\beta_j}$ and $\dt{\alpha} = \max_{j\in T} \dt{\beta_j}$. Therefore, $k\dt{\beta_{p_i}} + \dt{\gamma} = k\dt{\alpha} + \dt{\gamma} \geq 0$, since
			we couldn't decrease dual anymore. Now using \eqref{eq:beta-change}, we know that $\dt{\beta_{p_i}} = f_{\ALG^{(i)}}(p_i) - \beta_{p_i}$. Rearranging gives us \eqref{eq:main}. 
			
			Next, we use the fact that $p_i \in T$ to deduce $\beta_{p_i} = \alpha$, and use \eqref{eq:gamma-change} to note $\dt{\gamma} = f(\ALG^{(i)}) - \gamma$. Substituing above, we get
			\[
			f(\ALG^{(i+1)}) - f(\ALG^{(i)}) = f_{\ALG^{(i)}}(p_i)  \geq \alpha - \frac{f(\ALG^{(i)} - \gamma)}{k} 
			\]
			rearranging which implies
			\begin{equation}
				f(\ALG^{(i+1)}) \geq \left(1 - \frac{1}{k}\right) f(\ALG^{(i)}) + \frac{1}{k}\cdot \dual
			\end{equation}
			Since $\dual$ just before $i$th item is picked is only at least the final dual objective (since we only decrease dual).~\Cref{clm:ana} gives us the theorem.
		\end{proof}
		
		\subsection{Discretization and Reformulation}\label{sec:discrete}
		
		In this step we describe the discrete reformulation of the continuous algorithm described above, especially the lines~\ref{alg:mdp-first} to~\ref{alg:mdp-last}. To this end, 
		suppose we have just added $p_i$ to $\ALG^{(i)}$ in Line~\ref{alg:16}, and the resulting $\dt{\gamma}$ and $\dt{\alpha}$ calculated in Line~\ref{alg:17} and Line~\ref{alg:19}, respectively,
		satisfy $k\dt{\alpha} + \dt{\gamma} < 0$. This is when we enter the inner while-loop and run lines~\ref{alg:mdp-first} to~\ref{alg:mdp-last}.
		Let this be $t=0$ and let all variables and their rates be in indexed by this time, that is, $\alpha(0) = \alpha$, $\dt{\alpha}(0) = \dt{\alpha}$, and so on and so forth.
		We also let $T(0)$ denote the tight set at this point. 
		%Crucially note: the element just added $p_i \in T(0)$ since it was picked from a tight set and Lines~\ref{alg:16} to~\ref{alg:19} do not modify$\alpha, \beta_j, \gamma$'s (only the rates) and thus $T$ is unchanged. Furthermore, $\dt{\alpha}(0) = 1$
		
		
		We now explain evolution of these various variables as a function of $t$ while we are in the inner while-loop. Since $\calA$ and $\ALG$ don't change in the inner while loop all the rates behave in a predictable manner which will allow us to ``shortcut'' the inner while loop. We discuss this, and then describe the discrete algorithm.
		
		For brevity's sake, we use $F:= f(\ALG)$ and $F_j := f_{\ALG}(j)$ for all $j\in V$. The variable $\dt{\beta}_j(t)$ behaves as per the ordinary differential equation
		\begin{equation}\label{eq:beta-evol}
			\forall j \in V,~~~ \dt{\beta_j}(t) = F_j - \beta_j(t) ~~\Rightarrow~~~~~ \beta_j(t) = \beta_j(0)\cdot e^{-t} + F_j\cdot (1-e^{-t}) ~~\textrm{and}~~ \dt{\beta}_j(t) = \dt{\beta}_j(0)\cdot e^{-t}
		\end{equation}
		Similarly, we get the evolution of $\gamma(t)$ and $\dt{\gamma}(t)$ as 
		\[
		\dt{\gamma}(t) = F - \gamma(t)~~\Rightarrow~~~~~ \gamma(t) = \gamma(0)\cdot e^{-t} + F\cdot (1-e^{-t})~~~\textrm{and}~~~ \dt{\gamma}(t) = \dt{\gamma}(0)\cdot e^{-t}
		\]
		That is, the $\beta_j$ (and $\gamma$) variables are a convex combinations of $F_j$ (of $F$) and their old values. Crucially note that the ratio $\dt{\beta}_j(t)/\dt{\gamma}(t)$ is unchanged over time
		and is the original $\dt{\beta_j}(0)/\dt{\gamma}(0)$.
		
		Next, note that the value of $\dt{\alpha}(t) = \max_{j\in T(t)} \dt{\beta}_j(t)$ and thus equals $\dt{\beta}_{j_t}(t)$ for some ${j_t}\in T(t)$. Therefore, while $T(t)$ remains the same,
		the rate $\dt{\alpha}(t) = \dt{\beta}_{j_t}(t)$, and thus using the previous paragraphs argument, $\dt{\alpha}(t)/\dt{\gamma}(t)$ remains the same. In particular, till $T(t)$ changes,
		the while condition holds.
		
		Now note that until a new element is {\em added} to $T(t)$, the limiting $j_t$ never leaves $T(t)$, since $\beta_{j_t}(t)$'s rate of change and $\alpha$'s rate of change is the same as $\alpha(t)$'s rate of change.  Therefore, $\dt{\alpha}(t)$ changes {\em only} when a new element $\ell\notin T(t)$ is added to $T(t)$ whose $\dt{\beta}_\ell(t) > \dt{\beta}_{j_t}(t)$. At that instant, the value of $\dt{\alpha}(t)$ is set to $\dt{\beta}_\ell(t)$. At this point, we may have to check the while-loop condition.
		
		But we can {\em pre-compute} the set of element $\ell$ which would lead to a violation of the while-loop condition. This is again because the ratio $\dt{\beta}_\ell(t)/\dt{\gamma}(t)$ remains the same throughout. In particular, define the set 
		\[
		W := \{j \in ~V~: k\dt{\beta}_j(0) + \dt{\gamma}(0) \geq 0\} ~\underbrace{=}_{\text{since $\dt{\beta}_j(t)/\dt{\gamma(t)}$ remains unchanged}}~~~ \{j \in ~V~: k\dt{\beta}_j(t) + \dt{\gamma}(t) \geq 0\}
		\]
		where $\beta_j$ and $\gamma$ are values at time $0$. For a sanity check, note that $W$ doesn't contain a tight element since $\dt{\alpha} = \max_{j\in T} \dt{\beta}_j$ and if there was an intersection we would violate the inner while loop condition. The discussion preceding the set definition leads us to conclude that the inner while loop terminates the first time $t$ when an element in the set $W$ enters the set $T(t)$. Next, let's figure out the time when an element $\ell$ not in the tight set enters it. \smallskip
		
		Fix an element $\ell \notin T(0)$ and let $\dt{\alpha}(0) = \dt{\beta}_{j_0}(t)$ for $j_0 \in T(t)$. If these were the only two elements, then we can find the $t$ at which $\ell$ would enter 
		$T(t)$ by simply using \eqref{eq:beta-evol} on $\ell$ and $j_0$. Namely,
		\[
		\beta_\ell(t)e^{-t} + F_\ell(1- e^{-t}) = \beta_{j_0}(t) e^{-t} + F_{j_0}(1 - e^{-t}) ~~\Rightarrow ~~~ t_\ell  = \ln\left(1 + \frac{\beta_{j_0} - \beta_\ell}{F_\ell - F_{j_0}}\right)
		\]
		
		In particular, the first $\ell \notin T(0)$ which enters $T(t)$ is the element with minimum $t_\ell$, namely
		\begin{equation}
			\ell = \arg \max_{j\notin T(0)} \left(\frac{F_{j} - F_{j_0}}{\beta_{j_0} - \beta_j}\right) ~~~=:j_1 \label{eq:discrete-ell}
		\end{equation}
		So, $\ell$ is the element whose marginal increase on $\ALG$ is larger than $j_0$'s, but the algorithm shades this by the denominator which is the difference of the $\beta$-values.
		At time $t_\ell$, this element $\ell$ enters the tight set at time $t = t_\ell$ and, as discussed before, $\dt{\alpha}(t)$ increases to $\dt{\beta}_\ell(t)$. If $\ell \in W$, the inner while loop terminates. Otherwise, we again use equation \ref{eq:discrete-ell} to find the next element to become tight with the only change being that $\ell$ takes the value of ``$j_0$'' as the element which dictates $\dt{\alpha}_t$. This process continues till we find a $W$-element. We write the pseudocode below.
		
		\begin{center}
			\fbox{%
				\begin{varwidth}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
					%\begin{algorithm}[H]
						%	\caption{Continuous Dual Algorithm}
						\begin{algorithmic}[1]
							\Procedure{Discrete Make Dual Progress}:
							\LineComment{Replaces Lines~\ref{alg:mdp-first} to~\ref{alg:mdp-last} in Continuous Algorithm} 
							\LineComment{Below, we use $F_j := f_{\ALG^{(t)}}(j)$ for all $j$ and $F := f(\ALG^{(t)})$ for brevity}
							\State $j^* \eq \arg \max_{j\in T} \dt{\beta_j}$.
							\State $\ell \eq \arg \max_{j\in V\setminus T} \left(\frac{F_j - F_{j^*}}{\beta_{j^*} - \beta_j}\right)$ \Comment{Will enter $T$ next} \label{alg:5}
							\State $t \eq \ln\left(1 + \frac{\beta_{j^*} - \beta_\ell}{F_\ell - F_{j^*}}\right)$
							\State $\forall j \in V, \beta_j \eq \beta_j e^{-t} + F_j(1-e^{-t})$; $\dt{\beta_j} \eq F_j - \beta_j = \dt{\beta_j}e^{-t}$.
							\State $\gamma \gets \gamma e^{-t} + F(1 - e^{-t})$; $\dt{\gamma} \eq F - \gamma = \dt{\gamma}e^{-t}$.
							\State $\alpha \eq \beta_\ell e^{-t} + F_\ell (1-e^{-t})$.
							\State $T \gets \{{j \in V \mid \beta_j = \alpha}\}$ \Comment{$\ell$ enters $T$}
							\State If $\ell \in W$, then {\bf break}, else $j^* \eq \ell$ and go to line~\ref{alg:5}%$\dt{\alpha} \gets \dt{\beta}_\ell$\Comment{At this point $k\dt{\alpha} + \dt{\gamma} < 0$ needs to be checked.}
							\EndProcedure
						\end{algorithmic}					
						%	\end{algorithm} 
				\end{varwidth}%
			}
		\end{center}
		
		
		\paragraph{Query and Runtime Analysis.} 
		The number of queries is clearly $O(nk)$ since to make the algorithm run we need $f_{\ALG^{(t)}}(j)$ for all $j\in V$, and there are $k$ different sets.
		The running time is dominated by {\sc Discrete Make Dual Progress}. Naively, to find the element $\ell$ in Line~\ref{alg:5}, one can take $O(n)$ time, and 
		since any element can enter $T$ only once, this gives an $O(n^2)$ time for this procedure, and a total time of $O(kn^2)$ overall. 
		On the other hand, the operation in Line~\ref{alg:5} is trying to find an element which maximizes a ratio of two numbers, and after a change, both these numbers are 
		modified by subtracting the same value for each element. That is, the relative order of the elements as per the numerator and denominator remains the same. 
		The order related to the ratios can change and so this doesn't immediately imply an $O(n)$-time procedure, but it's possible the naive running time could be improved.
		We leave the exploration of this to the full version of this extended abstract which will discuss experimental results.
		
		At this point, the reader may wonder about the differences between the primal-dual algorithm and the greedy algorithm. We discuss this in \Cref{sec:greedy-comp}.
